Deep Episodic Memory: Encoding, Recalling, and Predicting Episodic Experiences for Robot Action Execution

We present a novel deep neural network architecture for representing robot experiences in an episodic-like memory which facilitates encoding, recalling, and predicting action experiences. Our proposed unsupervised deep episodic memory model 1) encodes observed actions in a latent vector space and, based on this latent encoding, 2) infers most similar episodes previously experienced, 3) reconstructs original episodes, and 4) predicts future frames in an end-to-end fashion. Results show that conceptually similar actions are mapped into the same region of the latent vector space. Based on these results, we introduce an action matching and retrieval mechanism, benchmark its performance on two large-scale action datasets, 20BN-something-something and ActivityNet and evaluate its generalization capability in a real-world scenario on a humanoid robot.

==> content/discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion}
Our approach is inspired by the composite encoder-decoder architecture proposed by \cite{Srivastava2015}. However, their approach is solely based on fully-connected LSTMs and thus only able to process low-resolution ($32\times32$) image patches or high-level representations of a pre-trained CNN. In contrast, our multi-layered convolutional LSTM architecture leverages both spatial and temporal weight sharing which makes it possible to process frame sequences with significantly higher resolution. Beyond benchmarking the latent representations as features for activity recognition, we show that videos of the same class tend to be mapped into the same region of the latent space. This property facilitates the use of simple machine learning classifiers (e.g. logistic regression or linear SVM) on top of the latent representations. Since these classifiers require significantly less training data than neural network based classifiers, activity and scene understanding problems in robotics, for which no comprehensive data set is available, could be solved in such way.

The proposed matching and retrieval mechanism in the latent space resembles episodic memory-like capabilities such as the recollection of previously experienced visual episodes. However, in our experiments, there are no temporal dependencies between the visual episodes within the memory since we use temporally independent data. We argue, that the temporal dependencies are introduced while the robot sequentially experiences its own episodes when interacting with its environment.






==> content/model.tex <==
\subsection{Model}
Especially with regard to videos, the lack of comprehensively labelled data sets makes supervised training difficult. Therefore, a first step towards learning to understand actions in videos are future frame prediction models. To successfully predict future video frames, such models are forced to generate latent representations of the inherent structure and dynamics of videos. In order to encode a visual experience into a representation vector of a latent space, we make use of frame prediction models and adopt the composite encoder-decoder architecture proposed in \cite{Srivastava2015} and in addition, introduce some modifications to it. The model, which conceptually combines an autoencoder with future frame prediction, consists of one encoder and two decoders. 

In our work, a visual experience is represented as a sequence of video frames $X=\{X_r \cup X_p\}=x_1,..,x_i \cup x_{i+1},...,x_{i+j}$. The encoder $E$ processes the sequence $X_r=x_1,..,x_i$ and projects it into a latent vector space of visual experiences with $I=E(X_r)$, yielding a representative of the frame sequence as a single latent vector $I$ within that space.

Subsequently, $I$ is forwarded to both decoders independently. The reconstruction-decoder $D_{rec}$ recovers the frames that were provided to $E$, giving us $X_r$ in reversed order, while the prediction-decoder $D_{pred}$ attempts to predict the future frames $X_p$. It is important to note that for determining the reconstruction and prediction error during training, both image sequences $X_r$ and $X_p$ are used, however, during test time only $x_i$ is provided to the model. The full interplay and the architecture is illustrated in figure \ref{fig:model}. The core idea of this structure rests upon $I$ being the only linkage between $E$ and both $D_{rec}$ and $D_{pred}$. Since input reconstruction as well as future prediction are performed based on this single representation vector, both $D_{rec}$ and $D_{pred}$ and more importantly $E$, are forced to conceptually contain all necessary information to reconstruct the input frames and model the future at the same time.
This information involves not just information about objects and the background but particularly the temporal dynamics of objects or actors. 

The input and output frames $x_i$ used in this work have a resolution of 128x128 pixels for each of the 3 color channels. Since Srivastava et al. use fully connected LSTMs, their model lacks to preserve spatial information throughout the process of encoding and decoding. Therefore, we exchange the vanilla LSTM layers with convolution LSTM layers\cite{Shi2015}, allowing us to also capture spatiotemporal correlations in the visual experiences. $E$ is therefore comprised of a stack of convolution LSTM and normal convolution layers (henceforth referred to as \emph{conv LSTM} and \emph{conv} layers) in alternating order. While the conv layers are operated with a stride of 2 in order to reduce the spatial size of the feature maps, the conv LSTM layers preserve the spatial size and forward information to the next time step through their hidden state and cell state. After the alternating series of conv and conv LSTM layers in the encoder, we add one fully convolutional and one fully convolutional LSTM layer $f_d(\cdot)$ to the stack. The former is required to due to dimension incompatibility between conv LSTM and fully conv LSTM while $f_d(\cdot)$ allows for practical variability of the latent representation dimensionality $d$, which can be controlled by the number of units $d/2$ in the layer.

With $f_d(\cdot)$ being the last layer of $E$, it yields two output vectors, each of having the dimensionality $d/2$. The hidden state vector $H_{d/2}$ and cell state vector $C_{d/2}$ are composed to $(H_{d/2}, C_{d/2})$, producing the final latent representation $I_d$ that is passed on to the decoders. Both decoders have the inverted structure of the encoder, meaning that transposed convolution layers are used to increase the spatial size of the feature maps throughout the decoding layers until the full video frame resolution of 128x128 is reached. 

As loss functions we used $L2$ reconstruction loss (equation \ref{eq:l2}) and Image Gradient Difference Loss from \cite{Mathieu2015} (equation \ref{eq:gdl}) in our experiments.

\begin{equation}
L2 = \frac{1}{2N}\sum_{n=1}^{N}\lVert{x'_n - x_n}\lVert^2
\label{eq:l2}
\end{equation}

\begin{equation}
\begin{split}
GDL = \sum_{n=1}^{N}\sum_{i,j}\lVert\lvert x_{n_{i,j}} - x_{n_{i-1,j}} \rvert - \lvert x'_{n_{i,j}} - x'_{n_{i-1,j}}\rvert\rVert +\\ \lVert\lvert x_{n_{i,j-1}} - x_{n_{i,j}} \rvert - \lvert x'_{n_{i,j-1}} - x'_{n_{i,j}}\rvert\rVert
\end{split}
\label{eq:gdl}
\end{equation}

The loss is computed over all ground truth frames $x_n$ and the frames $x'_n$ generated by $D_{rec}$ and $D_{pred}$. Since squared loss shows instabilities to small image deformations and is prone to linear blurring as identified by Ranzato et. al\cite{Ranzato2014}, we also ran experiments with GDL and a weighted combination of both. Acting on an image gradient level, the GDL function directly penalizes differences between the gradients of the predicted frame and the ground truth frame. 

%(!!!add alpha to gdl equation? we used alpha=1!!!)

We trained the network with the adaptive learning rate method ADAM\cite{Kingma2014a} in conjunction with a exponentially decaying learning rate schedule. Weight updates were conducted with Stochastic Gradient Descent (SGD) and a batch size of 50 training samples.
On each network layer except the last encoder layer (\emph{since it is our output layer}), we used layer normalization\cite{Ba2016} and dropout with dropout probabilities between 10\% and 15\%. 
% (reference to experiments might be required here).

% noise

During the training and validation process different variations of the described network architectures were used. Table \ref{table:models} depicts the different model variations and lists the layers of which they are composed of.  

\begin{table*}
\centering
\begin{tabular}{l|cccccccccccc}
Model                    & \begin{turn}{90} conv1\end{turn} & \begin{turn}{90} conv LSTM1\end{turn} & \begin{turn}{90} conv2\end{turn} & \begin{turn}{90} conv LSTM2\end{turn} & \begin{turn}{90} conv3\end{turn} & \begin{turn}{90} conv LSTM3\end{turn} & \begin{turn}{90} conv4\end{turn} & \begin{turn}{90} conv LSTM4\end{turn} & \begin{turn}{90} conv5\end{turn} & \begin{turn}{90} conv LSTM5\end{turn} & \begin{turn}{90} FC Layer Size\end{turn}  & \begin{turn}{90} FC LSTM Size\end{turn} \\ \hline
4 conv/conv LSTM          & 5x5   & 5x5       & 5x5   & 5x5       & 3x3   & 3x3       & 3x3   & 3x3       &       &           &     &        \\
4 conv/conv LSTM + FC $n$   & 5x5   & 5x5       & 5x5   & 5x5       & 3x3   & 3x3       & 3x3   & 3x3       &       &           & $n$   &        \\
5 conv/conv LSTM          & 5x5   & 5x5       & 5x5   & 5x5       & 5x5   & 3x3       & 3x3   & 3x3       & 3x3   & 3x3       &     &        \\
5 conv/conv LSTM + FC $n$   & 5x5   & 5x5       & 5x5   & 5x5       & 5x5   & 3x3       & 3x3   & 3x3       & 3x3   & 3x3       & $n$   &        \\
5 conv/conv LSTM + FC LSTM $n$ & 5x5   & 5x5       & 5x5   & 5x5       & 5x5   & 3x3       & 3x3   & 3x3       & 3x3   & 3x3       & $2n$ & $n$     
\end{tabular}
\caption{Models used during training - Layers from encoder input (left) to output (right). For conv and conv LSTM layers the filter size $kxk$ is provided whereas fully connected (FC) layers and fully connected LSTM are characterized by their layer size $n$. \label{table:models}}
\end{table*}



